Glucose-insulin mathematical model for the combined effect of medications and life style of Type 2 diabetic patients

The goal of this paper is to propose a new mathematical model for the combined effect of different treatments and lifestyles on the glucose-insulin dynamics of Type 2 diabetes (T2D) patients. The model gives the possibility to take into consideration physical activity, stress, meals, and medications while evaluating or designing treatment plans for T2D patients. The model is proposed by combining and modifying some of the available models in the literature. Simulations were performed for the modifications to show how the model confirm with literature on T2D patients. Additionally, a discussion is provided to demonstrate the ability of the model to be used in the assessment of treatment plans and in the design for robust insulin dose guidance algorithms. An open source code for the model is additionally provided.

==> trash.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
         $V^{G}_{BC}~\si{[dL]}$ & 3.5 & $V^{G}_{BF}~\si{[dL]}$ & 4.5 & $V^{G}_{H}~\si{[dL]}$ & 3.5 & $V^{G}_{L}~\si{[dL]}$ & 25.1\\
         \hline
         $V^{G}_{G}~\si{[dL]}$ & 11.2 & $V^{G}_{K}~\si{[dL]}$ & 6.6 & $V^{G}_{PC}~\si{[dL]}$ & 10.4 & $V^{G}_{PF}~\si{[dL]}$ & 67.4 \\
         \hline
         $V^{I}_{B}~\si{[L]}$ & 0.26 & $V^{I}_{H}~\si{[L]}$ & 0.99 & $V^{I}_{G}~\si{[L]}$ & 0.94 & $V^{I}_{L}~\si{[L]}$ & 1.14\\
         \hline
         $V^{I}_{K}~\si{[L]}$ & 0.51 & $V^{I}_{PC}~\si{[L]}$ & 0.74 & $V^{I}_{PF}~\si{[L]}$ & 6.74 & $V^{\Gamma}~\si{[mL]}$ & 6.74\\
         \hline
         $Q^{G}_{B}~\si{[dL\,min^{-1}]}$ & 5.9 & $Q^{G}_{H}~\si{[dL\,min^{-1}]}$ & 43.7 & $Q^{G}_{A}~\si{[dL\,min^{-1}]}$ & 2.5 & $Q^{G}_{L}~\si{[dL\,min^{-1}]}$ & 12.6\\
         \hline
         $Q^{G}_{G}~\si{[dL\,min^{-1}]}$ & 10.1 & $Q^{G}_{K}~\si{[dL\,min^{-1}]}$ & 10.1 & $Q^{G}_{P}~\si{[dL\,min^{-1}]}$ & 12.6 & $Q^{I}_{B}~\si{[dL\,min^{-1}]}$ & 0.45 \\
         \hline
         $Q^{I}_{H}~\si{[L\,min^{-1}]}$ & 3.12 & $Q^{I}_{A}~\si{[L\,min^{-1}]}$ & 0.18 & 
         $Q^{I}_{K}~\si{[L\,min^{-1}]}$ & 0.72 & $Q^{I}_{P}~\si{[L\,min^{-1}]}$ & 1.05 \\
         \hline
         $Q^{I}_{G}~\si{[L\,min^{-1}]}$ & 0.72 & $Q^{I}_{L}~\si{[L\,min^{-1}]}$ & 0.9 & $T^{G}_{B}~\si{[min]}$ & 2.1 & $T^{G}_{P}~\si{[min]}$ & 5.0\\ 
         \hline
         $T^{I}_{P}~\si{[min]}$ & 20.0 & $f_{q}~\units{\cdot}$ & 0.9 &
         $k_{\phi1}$ & 0.68 & $k_{\phi2}$ & 0.00236\\
         \hline
         $k_{12_{q}}~\si{[min^{-1}]}$ & 0.08 & $k_{\mathrm{min}}~\si{[min^{-1}]}~\si{[min^{-1}]}$ & 0.005 & $k_{\mathrm{max}}~\si{[min^{-1}]}$ & 0.05 & $k_{\mathrm{abs}}~\si{[min^{-1}]}$ & 0.08\\
         \hline
         $c^{I}_{PGU}~\units{\cdot}$ & 0.067 & $c^{I}_{HGP\infty}~\units{\cdot}$ & 1.59 & $c^{G}_{HGP}~\units{\cdot}$ & 0.62 & $c^{I}_{HGU\infty}~\units{\cdot}$ & 1.72\\
         \hline
         $c^{G}_{HGU}~\units{\cdot}$ & 2.03 & $d^{I}_{PGU}~\units{\cdot}$ & 1.126 & $d^{I}_{HGP\infty}~\units{\cdot}$ & 0.683 & $d^{G}_{HGP}~\units{\cdot}$ & 0.14\\
         \hline
         $d^{I}_{HGU\infty}~\units{\cdot}$ & 0.023 & $d^{G}_{HGU}~\units{\cdot}$ & 1.59 & $m_{l_{0}}~\si{[U]}$ & 6.33 & $\zeta_{1}~\si{[L\,pmol^{-1}]}$ & 0.0026\\
         \hline
         $\zeta_{2}~\si{[L\,(pmol\,min)^{-1}]}$ & $0.99\text{e}^{-4}$ & $K_{l}~[\si{min^{-1}}]$ & 0.3621 & $K_{s}~[\si{min^{-1}}]$ & 0.0572 & $\gamma~\units{\mu g\,min^{-1}}$ & 2.366\\
         \hline
         $\alpha~\units{min^{-1}}$ & 0.615 & $\beta~\units{min^{-1}}$ & 0.931 & $N_{1}~\units{min^{-1}}$ & 0.0499 & $N_{2}~\units{min^{-1}}$ & 0.00015\\
         \hline
         $V^{\Psi}~\units{dL}$ & 11.31 & $K_{out}~\units{min^{-1}}$ & 68.3041 & $\mathit{Cf}_{2}~\units{min^{-1}nmol^{-1}}$ & 21.1512 & $\tau_{\psi}~\units{min^{-1}}$ & 35.1\\
         \hline
         $R_{maxC}~\units{nmol}$ & 5.0 & $\zeta~\units{\cdot}$ & 8.248 & $f_{v}~\units{\cdot}$ & 0.772 & $k_{a1}~\units{min^{-1}}~\units{min^{-1}}$ & 0.021\\
         \hline
         $k_{a2}~\units{min^{-1}}$ & 0.0175 & $\mathit{CL}~\units{L\,h^{-1}}$ & 0.6067 & $\mathit{CL}_{\mathit{ic}}~\units{L\,h^{-1}}$ & 0.6683 & $V_{p}~\units{L}$ & 97.3\\
         \hline
         $k_{off}~\units{h^{-1}}$ & 0.0102 & $R_{maxP}~\units{nmol}$ & 13 & $k_{deg}~\units{h^{-1}}$ & 0.0018 & $V_{c}~\units{L}$ & 22.2\\
         \hline
         $K_{vd}~\units{nmol\,L^{-1}}$ & 71.9 & $k_{v2}~\units{h^{-1}}$ & 0.39 & $k_{go}~\units{min^{-1}}$ & $1.88\text{e}^{-4}$ & $k_{gg}~\units{min^{-1}}$ & $1.85\text{e}^{-4}$\\
         \hline
         $k_{pg}~\units{min^{-1}}$ & 4.13 & $k_{gl}~\units{min^{-1}}$ & 0.46 & $k_{pl}~\units{min^{-1}}$ & 0.00101 & $k_{lp}~\units{min^{-1}}$ & 0.91\\
         \hline
         $k_{po}~\units{min^{-1}}$ & 0.51 & $\nu_{G W, \max }~\units{\cdot}$ & 0.486 & $\nu_{L, \max }~\units{\cdot}$ & 0.378 & $\nu_{P, \max }~\units{\cdot}$ & 0.148\\
         \hline
         $n_{GW}~\units{\cdot}$ & 2.0 & $n_{L}~\units{\cdot}$ & 2.0 & $n_{P}~\units{\cdot}$ & 5.0 & $\phi_{GW, 50 }~\units{\cdot}$ & 431.0\\
         \hline
         $\phi_{L, 50 }~\units{\cdot}$ & 521.0 & $\phi_{P, 50 }~\units{\cdot}$ & 1024.0 & $\rho_{\alpha}~\units{min^{-1}}$ & 54 & $\rho_{beta}~\units{min^{-1}}$ & 54\\
         \hline
         $\alpha_{M}~\units{min^{-1}}$ & 0.06 & $\beta_{M}~\units{min^{-1}}$ & 0.1 & $p_{la}~\units{min^{-1}}$ & 0.5 & $r_{la}~\units{\cdot}$ & 0.2143\\
         \hline
         $q_{la}~\units{dL^2\,mU^{-2}}$ & $3.04\text{e}^{-10}$ & $b_{la}~\units{min^{-1}}$ & 0.025 & $C_{\mathrm{max}}$ & 15.0 & $k_{la}~\units{min^{-1}}$ & $2.35\text{e}^{-5}$\\
         \hline
         $p_{fa}~\units{min^{-1}}$ & 0.5 & $r_{fa}~\units{\cdot}$ & 0.2143 & $q_{fa}~\units{dL^2\,mU^{-2}}$ & $1.3\text{e}^{-11}$ & $b_{fa}~\units{min^{-1}}$ & 0.0068\\
         \hline
         $\tau_{\mathit{HR}}~\units{min}$ & 5.0 & $n_{e}~\units{\cdot}$ & 4.0 & $a_{e}~\units{\cdot}$ & 0.1 & $\tau_{e}~\units{min}$ & 600\\
         \hline
         $\alpha_{e}~\units{\cdot}$ & 2.974 & $\beta_{e}~\units{bpm^{-1}}$ & $3.39\text{e}^{-4}$ & & & &\\
         \hline
         
    \end{tabular}
     \captionsetup{aboveskip=0pt,font=it}    \caption{Parameters Values}
    \label{tab:Param}
    In this section, simulation results for different cases are included to discuss the modified model. The model was implemented in Matlab and the software can be obtained upon request from one of the authors. The parameters are taken to be mean parameters from the corresponding literature for the different models except for $\alpha_e$ that was tuned to make the response similar to the one in \cite{Breton2008}. The values of the parameters can be found in appendix \ref{sec:param}.
All the simulation cases start with initial condition of $G_{PC}(0)=10~\units{mmol\,L^{-1}}$ for glucose concentration in the central periphery compartment and $I_{PF}=1~\units{mU\,L^{-1}}$ for the insulin concentration in the interstitial fluid periphery compartment. The patient is assumed to be having three meals each day with a corresponding glucose net amount of $5~\units{g}$ for the first meal, $5~\units{g}$ for the second meal, and $50~\units{g}$ for the third meal.
\subsection{Insulin Injection}
For this case, the patient is assumed to be taken a Glargin long acting insulin dose of $30~\units{U}$ each morning and a Lispo fast acting insulin dose of $0.5~\units{U}$ at the same time for the third meal. The results are shown in Figure \ref{fig:Insulin}. The long acting insulin raise the level of insulin during the day in general and reduces glucose concentration in the same manner. The fast acting insulin raises the insulin levels for the third meal so it does not cause a large spike in glucose. The figure also shows the natural body insulin response to increases of glucose upon the consumption of meals where fast acting insulin is not injected. The natural body insulin response is seen clearly when the insulin rise in a more apparent manner in the plasma rather than the peripherals. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/Insulin.eps}
    \caption{Simulation results with insulin injections.}
    \label{fig:Insulin}
\end{figure}

\subsection{Metformin and Stress}
As for this case, the patient is assumed to be taking a metformin oral dose of $0.6~\units{\mu g}$ each morning without any insulin doses. However, the patient experiences stress with severity $\alpha_{s}=0.3$ during the second day of the simulation. The simulation results are shown in Figure \ref{fig:Stress}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/Stress.eps}
    \caption{Simulation results with Metformin oral doses and stress effect.}
    \label{fig:Stress}
\end{figure}
The Metformin effect can be seen especially in the last day. It decreases glucose concentration by enhancing the sensitivity to insulin. At the same time, the body naturally reduces its production of insulin. Additionally, it can be seen how stress can raise the glucose concentration and decrease insulin sensitivity.

\subsection{Metformin and Physical Activity}
For this simulation, the patient is exercising for an hour each day after three hours of the last meal in addition to the metformin medication. The exercise raises the heart rate by $30~\units{bpm}$ from a rest value of $40~\units{bpm}$ during the entire hour. Figure \ref{fig:PH} shows the results.
The effect of physical activity can be seen by an apparent decrease in the peripherals glucose concentration during the exercise followed by a prolonged effect that is caused by the enhancement of insulin action on glucose using the state $E_{2}$. The same effect is discussed in \cite{Breton2008}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/PH.eps}
    \caption{Simulation results with Metformin oral doses and physical activity.}
    \label{fig:PH}
\end{figure}


\end{table*}
